Using Word Embeddings for Automatic Query Expansion

In this paper a framework for Automatic Query Expansion (AQE) is proposed using distributed neural language model word2vec. Using semantic and contextual relation in a distributed and unsupervised framework, word2vec learns a low dimensional embedding for each vocabulary entry. Using such a framework, we devise a query expansion technique, where related terms to a query are obtained by K-nearest neighbor approach. We explore the performance of the AQE methods, with and without feedback query expansion, and a variant of simple K-nearest neighbor in the proposed framework. Experiments on standard TREC ad-hoc data (Disk 4, 5 with query sets 301-450, 601-700) and web data (WT10G data with query set 451-550) shows significant improvement over standard term-overlapping based retrieval methods. However the proposed method fails to achieve comparable performance with statistical co-occurrence based feedback method such as RM3. We have also found that the word2vec based query expansion methods perform similarly with and without any feedback information.

==> method-new.tex <==
\section{Word Embedding based Query Expansion}
\label{sec:method}
In this section, we first describe more precisely the basic, word embedding
based QE method outlined in the Introduction. Unlike pseudo relevance
feedback (PRF) based QE methods, this method does not require an initial
retrieval. The second approach we propose is inspired by
\cite{weston2014memory}, where the nearest neighbors are computed in an
incremental fashion as elaborated below. As a third alternative, we
consider a straightforward variation of the first approach that uses word
embeddings in conjunction with a set of pseudo relevant documents.

Recall that the basic principle behind word embedding based QE is to use
terms that are close to the query terms in the embedding space. However,
instead of considering terms that are proximate neighbours of individual
query words, it is generally preferable to consider terms that are close to
the query as a whole.\footnote{This idea has been used in a number of
  traditional, effective QE techniques, e.g., RM3.} Therefore, we need to
define a measure that captures the overall or \emph{composite} similarity
between a set of query terms $\{ q_1, q_2, \ldots, q_k \}$ and a candidate
expansion term. We describe below the method adopted in this study for
\emph{term composition}.

 below. 


\subsection{Composition of Terms}
\label{subsubsec:compose}
Consider the TREC query 301: \emph{International Organized Crime}. If we search 
for similar terms of the individual query terms (similar words of 
\emph{International}, \emph{Organized} and \emph{Crime}) we may end up 
with some new terms which are less associated to the actual information need. To 
achieve something more purposeful, it would be nice to have some expansion words 
which are related to the query as a whole (similar words of 
\emph{International Organized Crime}). As all the terms have a vector 
corresponding to it, we can easily get the effect of composition 
of query terms by composing the vectors corresponding to it. 
% For example, suppose $q_1, q_2$ are two query terms and $\overrightarrow{q_1}, 
% \overrightarrow{q_2}$ are the vectors corresponding to the terms. Among many 
% sophisticated techniques, one simple and easy to understand method is adding 
% the vectors: \\
% % \begin{center}
% %     $composed(q_1,q_2) = \overrightarrow{q_1} + \overrightarrow{q_2}$    
% \end{center}

\para{Deriving Composed Words}
Given a query of $k$ terms, $Q=\{q_1,\ldots,q_k\}$, we compose the vectors 
corresponding to the query words in a linear chain from left to right, i.e., 
for a $k$ term query, we obtain the set $q_c$, comprised of
$k-1$ composed query points, as shown in Equation \ref{eq:qc}.

\begin{equation}
Q_c = \bigcup_{i=1}^{k-1}(vec(q_i) + vec(q_{i+1}))  \label{eq:qc}
\end{equation} 
We consider only the linear chain composition of $q_i$ and $q_j$ from left to 
right instead of considering all possible combinations assuming coexisting terms 
(when $j-i=1$) give more meaningful composition than terms $q_i$ and $q_j$ 
with other words appearing in between them (when $j-i>1$).\\


\para{Extended Query term set}
\label{subsec:qe}
Following the proposed approach, for a given query $Q=\{q_1,\ldots,q_k\}$, the 
final extended query term set will take the following form: \\
\begin{equation}
    Q' = Q \cup Q_c    \label{eq:qe2}
\end{equation}



\subsection{Pre-retrieval Nearest Neighbor based approach for QE} \label{knn-pre}
The basic goal of query expansion techniques is to introduce new terms into the existing query to better reflect the information need. 
One major advantage of having embedded representations for words of the vocabulary, is that we can understand the semantic relationships between terms.
Thus, utilizing this semantic information, we develop a nearest neighbor based approach.
%For efficiency, these similar terms can be kept in memory. 
In our approach, we used \textit{word2vec} for finding these similar terms. \\
Formally, given a query, we obtain the extended query term set (EQTS) $Q'=\{q_1, \dots, q_k\}$ following the composition of terms method. The expansion terms for $Q'$ is determined based on the semantic similarity between the  candidate expansion term and each of the query terms and also the terms obtained by query term composition. From now on, in the rest of this section, by query terms, we will refer to composed terms in $Q_{c}$ in addition to terms in $Q$.

\para{Expanded Query}
Following the above approach, for a given query, the EQTS $Q'=\{q_1,\ldots,q_k\}$, the 
expanded form will be the following:\\
\begin{equation}
    Q_{exp} = \bigcup_{q\in Q'} NN(q)   \label{eq:qe1}
\end{equation}
where \emph{NN()} is a method that returns top $N$ terms which are similar 
to the vectors of the query terms.

The $Q_{exp}$ terms contains all the candidate expansion terms from which the final top $N$ terms are computed. For each candidate expansion term, the mean of the cosine similarity with all the terms in Q' is computed. This mean score is designated as the final similarity score and the top $N$ expansion terms are computed based on this score. $Q'_{exp}$ contains the top $N$ nearest neighbors after the above operations.



\subsection{Pre-retrieval incremental Nearest Neighbor based approach for QE} \label{knn-post}
The incremental nearest neighbor method, is a simple extension of the previous method. Instead of computing the nearest neighbor expansion term, for a query term, in a single step, we follow an incremental procedure. The first assumption in this method is that, the most similar expansion terms have comparatively lower drift than the terms occurring later in the list in terms of similarity. Since the top similar terms in the vocabulary are contender in becoming the expansion query terms, it can be assumed that these terms are also similar to each other, in addition to being similar to the query term.
Following the above assumption a iterative process pruning of terms from the vocabulary is done at each step for every the terms in EQTS. 
At the first step, we compute the nearest neighbors of the query term under consideration. We prune this set by a fixed amount $K$.
Next we consider the most similar term in the pruned nearest neighbor set and make it the query term and repeat the above procedure for a fixed $l$ number of steps.
At each step the nearest neighbors set is computed based on the nearest neighbor of the previous set and the set is pruned.
Essentially, by following the above procedure, we are constraining the nearest neighbor to be similar to each other in addition to being similar to the query term.
A high value of $l \geq 10$ may lead to risk of query drift. A low value of $l \leq 2$ essentially performs similar to normal pre-retrieval model. By careful tuning we choose  $l = 5$ as the number of iterations for this method.
After getting the nearest neighbor list for each term in EQTS, $Q_{exp}$ and $Q'_{exp}$ are computed following the same method as above.

\subsection{Nearest Neighbor based approach for QE with feedback} \label{knn-post}
Using relevance feedback for query expansion is empirically shown to be very effective.
In our third approach, we use pseudo-relevance feedback(PRF) to restrict the search domain for the candidate query terms.
Instead of searching the whole vocabulary, in this approach, we consider only those terms which occurs in top initially retrieved document. The number of documents to be used as PRF are varied as a parameter. The procedure to compute the expansion
query terms is same as in case of Pre-retrieval method. The only difference here is that, we are searching the nearest neighbors within the terms which occur in the pseudo-relevant documents.


\subsection{Retrieval}
\label{subsec:ret}
The expanded query is formed depending only on the original query terms ($Q$) and how they appear in 
the collection as a whole. Thus the actual retrieval can be done using any 
standard retrieval model. For our experiment, we used Language Model with 
Jelinek Mercer smoothing \cite{zhai}. Linear smoothing parameter $\lambda$ is 
tuned. The expansion term weights are assigned by normalizing the expansion term score (mean similarity with respect to all the terms in EQTS) by the total score obtained by summing over all top $N$ expansion terms. This weights are multiplied with $1- \lambda$ and added with the the original query scaled by $\lambda$ to give the expanded query.

$\Sum_{q\belongs}$

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "qe"
%%% End:


==> rel-work.tex <==
\section{Related Work}
\label{sec:rw}
% Clinical decision support: In \cite{GoodwinH14} query expansion is performed through neural langauge model (Word2Vec) in conjunction with query expansion through Wikipedia, United Medical Language System (UMLS) and he Systematized Nomenclature of Medicine Clinical Terms (SNOMED CT) . The motive behind the use of Word2Vec is to get more generic expansion terms, while domain specific terms are provided from UMLS and SNOMED CT 

% \cite{GrbovicDRSB15} proposed a method of task of query rewriting for finding similar queries and relevant ads to query issued. Three models are proposed, which are inspired from distributed language model for word and phrases. Model \emph{context2vec} tries to learn the semantic and temporal relationship between similar queries from search log. Model \emph{content2vec} is a modified version of paragraph2vec and tries to learn the word contained in the query (semantic relationship) and the query vector simultaneously. The paper also proposes a two layered joint model \emph{context-content2vec} which tries to incorporate the above two models in a single architecture.

% GLM

% Facebook: \cite{weston2014memory} suggest a novel memory network which acts as an efficient memory for information storage and act as an retrieval system for queries on the information stored. The embedding for the information are learned withing the network. 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "qe"
%%% End:

